A Hybrid Renewable-Battery-Electrolyzer Facility under the Single Imbalance Pricing Scheme

European energy markets are decentralized and entail balance responsibility of each market player. This stresses the importance of imbalance management of renewable energy sources (RES), as the imbalance payments can strongly reduce their profitability. According to the EU Electricity Balancing Guideline, each European transmission system operator should use the single imbalance pricing method which treats both deviation directions the same, no matter if a deviation helps the system or pushes it away from the balance. This paper aims to investigate the behavior of a hybrid facility consisting of an uncontrollable RES, a battery and an electrolyzer under such market setting. The formulated mathematical model of the hybrid facility seeks to maximize profit in the day-ahead energy market, while minimizing the imbalance costs. Uncertainty of the RES output is captured using stochastic scenarios, while the direction of the power system deviation, relevant for the imbalance pricing, is modeled using a newly proposed robust approach. Results of the case study indicate that the single imbalance pricing scheme might bring flexible assets to temptation of intentional deviations should they anticipate favorable imbalance prices.

==> nomenclature.tex <==
\section*{Nomenclature}
\addcontentsline{toc}{section}{Nomenclature}

\subsection{Abbreviations}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$\overline{P}^\mathrm{min}_{d}$, $\underline{P}^\mathrm{max}_{d}$}]
\item[BESS] Battery energy storage systems
\item[CIG] Converter-interfaced generation
\item[CHP] Combined heat \& power
\item[EC] Energy community
\item[EEC] Fully-electrified energy community
\item[EU] European Union
\item[FC]  Fuel cell
\item[GEC] Gas-based energy community
\item[HEC] Hydrogen-based energy community
\item[HP] Heat pump
\item[MG] Microgrid
\item[RES] Renewable energy sources
\item[RoCoF] Rate-of-change-of-frequency
\item[VSM] Virtual synchronous machine
\end{IEEEdescription}

\subsection{Superscripts}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$\overline{P}^\mathrm{min}_{d}$, $\underline{P}^\mathrm{max}_{d}$}]
\item[E/G/H/T] Electrical/Gas/Hydrogen/Thermal quantity
%\item[G] Gas quantity 
%\item[H] Hydrogen quantity
%\item[T] Thermal (heat) quantity
\end{IEEEdescription}

\subsection{Sets}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$\overline{P}^\mathrm{min}_{d}$, $\underline{P}^\mathrm{max}_{d}$}]
\item[$\mathcal{D}_m$] Set of all energy conversion devices in EC $m$
\item[$\mathcal{D}_{d,m}$] Set of devices $d\in \{ b, c, e, f, h, \beta, \tau, \hbar \}$ in EC $m$
\item[$\mathcal{D}^C_m$] Set of all energy conversion devices in EC $m$ that are not storage devices; $\mathcal{D}^C_m = \mathcal{D}_m \backslash \mathcal{D}^S_m$, $\mathcal{D}^C_m \subseteq \mathcal{D}_m$
\item[$\mathcal{D}^S_m$] Set of all energy conversion devices in EC $m$ that are also storage devices; $\mathcal{D}^S_m = \mathcal{D}_m\backslash \mathcal{D}^C_m$, $\mathcal{D}^S_m \subseteq \mathcal{D}_m$
\item[$\mathcal{M}$] Set of ECs, $\mathcal{M} = \{ \mathrm{EEC, GEC, HEC} \}$, indexed by $m$ 
\item[$\mathcal{N}_m$] Set of network nodes in EC $m$, indexed by $n$ 
\item[$\mathcal{T}$] Set of hours in a representative year, indexed by $t$
\end{IEEEdescription}

\subsection{Parameters}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$\overline{P}^\mathrm{min}_{d}$, $\underline{P}^\mathrm{max}_{d}$}]
\item[$E^\mathrm{max}_{d}$] Maximum state-of-energy of device $d$
\item[$E^\mathrm{min}_{d}$] Minimum state-of-energy of device $d$
\item[$L^\mathrm{E}_{n,m,t}$] Electric load demand at node $n$ in EC $m$ at time $t$
\item[$L^\mathrm{T}_{n,m,t}$] Heat demand at node $n$ in EC $m$ at time $t$
\item[$\overline{P}^\mathrm{max}_{d}$, $\underline{P}^\mathrm{max}_{d}$] Maximum input/ouput power of device $d$
\item[$\overline{P}^\mathrm{min}_{d}$, $\underline{P}^\mathrm{min }_{d}$] Minimum input/output power of device $d$
\item[$PV^\mathrm{E}_{n,m,t}$] PV production at node $n$ in EC $m$ at time $t$
\item[$\eta_d$] Energy conversion efficiency of device $d$
\item[$\eta^\mathrm{E}_d$] Electricity conversion efficiency of device $d$
\item[$\eta^\mathrm{T}_d$] Thermal conversion efficiency of device $d$
\item[$\eta^\mathrm{c}_d$] Charging efficiency of device $d$
\item[$\eta^\mathrm{d}_d$] Discharging efficiency of device $d$
\item[$\pi^\mathrm{E}_{t}$]{Electricity price at time $t$}
\item[$\pi^\mathrm{trans.}$]{Electricity transmission charge}
\item[$\pi^\mathrm{distr.}$]{Electricity distribution charge}
\item[$\pi^\mathrm{G}$]{Gas price}
\end{IEEEdescription}

\subsection{Variables}
\begin{IEEEdescription}[\IEEEusemathlabelsep\IEEEsetlabelwidth{$\overline{P}^\mathrm{min}_{d}$, $\underline{P}^\mathrm{max}_{d}$}]
\item[$\overline{p}_{d,m,t} $] Input power of device $d$ in EC $m$ at time $t$
\item[$\underline{p}_{d,m,t} $] Output power of device $d$ in EC $m$ at time $t$
\item[$x_{d,m,t} $] Binary variable indicating whether device $d$ in EC $m$ is operational at time $t$
\item[$x^\mathrm{c}_{d,m,t} $] Binary variable indicating whether device $d$ in EC $m$ is charging at time $t$
\item[$x^\mathrm{d}_{d,m,t} $] Binary variable indicating whether device $d$ in EC $m$ is discharging at time $t$
\item[$z_{d,m,t} $] Binary variable indicating whether device $d$ in EC $m$ has started up at time $t$
\item[$\gamma_{m}$] Gas volume bought from day-ahead market in EC $m$
\item[$\overline{\epsilon}_{m,t}$] Electricity volume bought from day-ahead market in EC $m$ at time $t$
\item[$\underline{\epsilon}_{m,t}$] Electricity volume sold to day-ahead market in EC $m$ at time $t$
\end{IEEEdescription}


